Optimal Sampling for Data Freshness: Unreliable Transmissions with Random Two-way Delay

In this paper, we aim to design an optimal sampler for a system in which fresh samples of a signal (source) are sent through an unreliable channel to a remote estimator, and acknowledgments are sent back over a feedback channel. Both the forward and feedback channels could have random transmission times due to time varying channel conditions. Motivated by distributed sensing, the estimator can estimate the real-time value of the source signal by combining the signal samples received through the channel and the noisy signal observations collected from a local sensor. We prove that the estimation error is a non-decreasing function of the Age of Information (AoI) for the received signal samples and design an optimal sampling strategy that minimizes the long-term average estimation error subject to a sampling rate constraint. The sampling strategy is also optimal for minimizing the long-term average of general non-decreasing functions of the AoI. The optimal sampler design follows a randomized threshold strategy: If the last transmission was successful, the source waits until the expected estimation error upon delivery exceeds a threshold and then sends out a new sample. If the last transmission fails, the source immediately sends out a new sample without waiting. The threshold is the root of a fixed-point equation and can be solved with low complexity (e.g., by bisection search). The optimal sampling strategy holds for general transmission time distributions of the forward and feedback channels. Numerical simulations are provided to compare different sampling policies.

==> sections/acknowledgment.tex <==
\section*{Acknowledgment}
This work has been supported in part by NSF grants: IIS-2112471, CNS-2106932, CNS-1901057, and CCF-1813050, and a grant from the Army Research Office: W911NF-21-1-0244.


==> sections/draft.tex <==
\begin{equation}

\end{equation}



\begin{proof}

\end{proof}


\begin{lemma}

\end{lemma}



\begin{align}

\end{align}


\Delta_{\text{opt}} 


 \mathbb{E} \left[   \right]

J_{\mu}

J_{\mu}(y)

Q_{\mu}(y,z)

\mathbb{P}(M_i >1)

\ \Bigg{|} \ 

\bar{z}

\textcolor{blue}{}

==> sections/problem_form.tex <==


%\title{Problem Formulation}
%	\title{Detection of Spatial Sparsity in Cognitive Radio Networks based on Compressive Sensing}


% \maketitle
% ------------------------------ ABSTRACT -----------------------------
\section{System Model}
\begin{figure}[t]
\includegraphics[scale=.5]{figures/Sys_mod.eps}
\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
\captionsetup{justification=justified}
\caption{System model.}
%\vspace{-.09in} 
 \label{sys_mod}
\end{figure}
We consider a remote estimation system as illustrated in Fig. \ref{sys_mod}, where a sensor takes samples from Ornstein-Uhlenbeck (OU) process $X_t$ and forwards the samples to an estimator via an error-free channel. Besides, the estimator has a continuous time noisy observation of the process $X_t$, called $O_t$. The error-free channel is modeled as a FCFS queue with i.i.d. service times. We suppose that there is an acknowledgement that is sent back to the sampler with zero delay whenever a sample is delivered. 

The System starts to operate at time $t=0$. We use $S_i$ to denote the generation time of the $i$-th sample, while $D_i$ denote  its delivery time to the estimator. Moreover, we use $Y_i$ to denote the service time of the $i$-th sample, where we have $0<\mathbb{E}[Y]<\infty$ and $D_i=S_i+Y_i$. Let $U(t)=\max{S_i:D_i\leq t}$ be the
sampling time of the latest received sample at time $t$. The age of information, or simply age, at time $t$ is defined as 
\begin{equation}
\Delta(t)=t-U(t).
\end{equation}
Since we have $D_{i}\leq D_{i+1}$, $\Delta(t)$ can be expressed as
\begin{equation}
\Delta(t)=t-S_i, \text{if}~t\in[D_i,D_{i+1}), i=0,1,2,\ldots
\end{equation}

The considered OU process  is defined as the solution to the following stochastic differential equation  (SDE)
\begin{equation}
dX_t=-\theta X_t dt+W_t,
\end{equation}
where $\theta>0$ is a parameter, and $W_t$ is a zero mean white noise process such that we have $\mathbb{E}[W_tW_s]=Q\delta(t-s)$ for all $0\leq t,s\leq\infty$. The observation process $O_t$ is modeled as 
\begin{equation}
O_t=HX_t+V_t,
\end{equation}
Where $H$ is some constant and $V_t$ is a zero mean white noise process such that we have $\mathbb{E}[V_tV_s]=R\delta(t-s)$ for all $0\leq t,s\leq\infty$.  We suppose that $W_t$ and $V_t$ are uncorrelated such that we have $\mathbb{E}[W_tV_s]=0$ for all $0\leq t,s\leq\infty$.

In this work, we use the Kalman filter \cite{ poor2013introduction} as the estimator. The Kalman filter provides an estimate $\hat{X}_t$ at time $t$. We aim to seek the optimal sampler that minimizes the mean-squared estimation (MSE) error $P_t\triangleq\mathbb{E}[(X_t-\hat{X}_t)^2]$  subject to an average sampling-rate constraint, which can be cast as the following problem:
\begin{align}
\text{mse}_\text{opt}=&\inf_{\pi\in\Pi}\limsup_{T\to\infty}\frac{1}{T}\mathbb{E}\left[\int_{0}^T P_t dt\right]\label{opt_eq5}\\&
\text{s.t.} \liminf_{n\to \infty}\frac{1}{n}\mathbb{E}\left[\sum_{i=1}^n (S_{i+1}-S_i)\right]\geq\frac{1}{f_\text{max}},\label{opt_eq6}
\end{align}
where $\text{mse}_\text{opt}$ is the optimum value of \eqref{opt_eq5}, $f_\text{max}$ is the maximum allowed sampling rate, and $\Pi$  represents the set of all causal sampling policies (some condition might be needed here such as regenerative condition, etc.). Note that the objective function in \eqref{opt_eq5} can be rewritten as (due to the regenerative property and renewal theory):
\begin{equation}
\limsup_{T\to\infty}\frac{1}{T}\mathbb{E}\left[\int_{0}^T P_t dt\right]=\limsup_{n\to\infty}\frac{\mathbb{E}\left[
\sum_{i=0}^n\int_{D_i}^{D_{i+1}} P_t dt\right]}{\mathbb{E}[D_n]}.
\end{equation}

The estimation process works as follows: The Kalman filter uses the continuous time observation $O_t$ to estimate the process $X_t$. Once a sample $i$ is delivered to the Kalman filter at time $D_i$, the Kalman filter re-initiate itself with the initial condition $P_{S_i}=0$ and starts a new estimation session. According to \cite{ poor2013introduction}, $P_t$ for $t
\in[D_i,D_{i+1})$ satisfies the following Riccati differential equation:
\begin{align}
\frac{dP_t}{dt}=-2\theta P_t+Q-\frac{H^2}{R}P_t^2.\label{rec_eqn}
\end{align}
Next, we derive a solution for Equation \eqref{rec_eqn} and show that $P_t$ is a non-decreasing function of the age process $\Delta(t)$.
\section{Main Results}
Let us define $\bar{P}$ as the steady state solution of \eqref{rec_eqn}, i.e., it is the solution of the following equation:
\begin{align}
0=-2\theta P_t+Q-\frac{H^2}{R}P_t^2.\label{rec_eqn_st}
\end{align}
Since our model is observable and controllable, we have $\bar{P}>0$. Hence, $\bar{P}$ is given by
\begin{align}
\bar{P}=\frac{-\theta R+\sqrt{(\theta R)^2+QRH^2}}{H^2}.
\end{align}
We derive $P_t$ in the next lemma.
\begin{lemma}\label{lim1}
For $t\in[D_i,D_{i+1})$ and $ i=0,1,2,\ldots$, the MSE $P_t$ is given by
\begin{align}
P_t=\bar{P}-\frac{1}{\frac{H^2}{2\sqrt{(\theta R)^2+QRH^2}}+\left(\frac{H^2}{-\theta R+\sqrt{(\theta R)^2+QRH^2}}-\frac{H^2}{2\sqrt{(\theta R)^2+QRH^2}}\right)e^{2\sqrt{\theta+Q\frac{H^2}{R}}\Delta(t)}}, \label{Lem1eq}
\end{align}
where $\Delta(t)=t-S_i$. Moreover, $P_t$ is a non-decreasing function of the age $\Delta(t)$.
\end{lemma}
\begin{proof}
See Appendix \ref{Appendix_A}.
\end{proof}
As a result of Lemma \ref{lim1}, we can use \cite{sun2017update} directly to solve our sampling Problem. Next, we show that when there is no side observation, i.e., $O_t=0$ for  $t\ge 0$, then our sampling problem reduces to the signal-agnostic sampling problem that is studied in \cite{ornee2019sampling}.
\begin{lemma}\label{Lim2}
When $O_t=0$ when $t\geq 0$, then the MSE $P_t$ for $t\in[D_i, D_{i+1})$ and $i=0,1,2 ,\ldots$ is given by
\begin{align}
P_t=\frac{Q}{2\theta}\left(1-e^{-2\theta\Delta(t)}\right).\label{Lim2_eq}
\end{align}
\end{lemma}
\begin{proof}
See Appendix \ref{Appendix_B}.
\end{proof}
Lemma \ref{Lim2} agrees with \cite[Lemma 4]{ornee2019sampling}.


%\bibliographystyle{IEEEbib}
%\bibliography{MyLib}
%\section{Appendix}
%\appendices





==> sections/related.tex <==
\section{Related Works}\label{related}

%    \begin{table} \caption{Comparing our study with related works} 
%\begin{center}  
%\begin{tabular}{|l|l|l|l|l|}
%\hline  
%  & \cite{arafa2020timely,klugel2019aoi} & \cite{tsai2021jointly,tsai2020age} & \cite{sun2017update, sun2019sampling,bedewy2019age} & Our Work \\ \hline
%Random Delay & \xmark &  \cmark  & \cmark & \cmark  \\
% \hline
%Two-way Delay & \xmark & \cmark  & \xmark & \cmark  \\
% \hline  
% Unreliable Channel & \cmark &  \xmark  & \xmark & \cmark \\
%   \hline  
%%Unbounded Forward Delay & \xmark & \xmark  & \cmark & \cmark \\
%% \hline
%\end{tabular}  
%\end{center} 
%\label{compare}
%\end{table}


%Our study is closely related to recent works in age of information, e.g., in \cite{kaul2012real,yates2015lazy,yates2021age,sun2017update,sun2019sampling,sun2017remote,arafa2020timely,tsai2021jointly,tsai2020age,ornee2019sampling,bedewy2019age,bedewy2021low,pan2021minimizing,pan2021minimizings,tsai2020unifying,zouminimizing,qian2020minimizing,bedewy2019agee,bedewy2019minimizing,sun2018age,klugel2019aoi}. In several different queuing systems, the Last-Generated, First-Served (LGFS) policy is shown to achieve age-optimality \cite{bedewy2019agee,bedewy2019minimizing,sun2018age}. Scheduling policies in various wireless networks are studied to minimize the age in e.g.,  \cite{bedewy2019age,bedewy2021low,pan2021minimizing,zouminimizing,qian2020minimizing}.   
%A literature review of the recent studies in age of information is provided in \cite{yates2021age}.  

Our paper is a contribution to the studies that design sampling policies to optimize data freshness metrics, e.g.,  \cite{yates2015lazy,sun2017update,sun2019sampling,arafa2020timely,tsai2020age,tsai2021jointly,bedewy2019age,klugel2019aoi}. 
%Regarding the channels setting, we compare our work with these studies in Table \ref{compare}.
%In \cite{yates2015lazy}, the authors state that to reduce the age, the source may need to wait before submitting a new sample. The study in \cite{sun2017update} generalizes the result in \cite{yates2015lazy}, proposes an optimal sampling policy under a Markov channel, and observes that the zero-wait policy is far from optimal if, for example, the transmission times are heavy-tail distributed or positively correlated.     
%In \cite{sun2019sampling}, the authors provide a survey of the age penalty functions that are related to autocorrelation, remote estimation, and mutual information. The optimal sampling solution is a deterministic or randomized threshold policy based on the objective value and the sampling rate constraint. However, the studies in \cite{sun2017update,sun2019sampling} assume reliable transmissions. Moreover, they consider a one-way transmission delay and ideally assume that the backward direction has a zero delay.       
%In \cite{tsai2020age}, the paper considers a two-way delay model and provides a low complexity algorithm with a quadratic convergence rate to compute the optimal threshold.  
%An optimal joint cost-and-AoI minimization solution is provided in \cite{tsai2021jointly} for multiple coexisting source-destination pairs with heterogeneous AoI penalty functions. 
 Our studies are different from that of \cite{tsai2021jointly,tsai2020age} in two aspects: (i) We generalize the channel condition of the forward direction to be time-varying. Besides, our study allows unbounded forward transmission times. (ii) 
% In \cite{tsai2021jointly,tsai2020age}, the papers assume that the age penalty function is continuous and the forward channel is bounded. 
The age penalty function in our study does not need to be continuous or positive. %which complies with some applications for periodic inspection and monitoring \cite{sun2017update}.
% and we only require the forward channel delay to have a finite expectation. 
%In \cite{arafa2020timely}, the authors assume a  
While most past works in optimizing sampling consider reliable transmissions, the studies in \cite{arafa2020timely,klugel2019aoi} are the exceptions that consider an unreliable forward channel, but with a constant one-way delay. 
In \cite{arafa2020timely}, the authors utilize convex optimization to solve the optimal sampling policy. However, using convex optimization is incorrect (even for a constant delay) if we allow the sampling policy to be randomized. In \cite{klugel2019aoi}, the authors choose \emph{idle} or \emph{transmit} at each time slot to minimize joint age penalty and transmission cost. The optimality of a threshold-based policy is shown, and the threshold of the policy is computed efficiently. Nevertheless, the technique of \cite{klugel2019aoi} is infeasible in our study since we consider an enlarged action space and random channel delays.  
%when the cost is neglected, it is optimal to always transmit a packet than staying idle since both the sampling time period and channel delay are one time slot.
%Nevertheless, the setting of one-way constant delay restricts the generality of their optimal sampling policies.         


%Finally, our paper contributes to establishing a new connection between remote estimation (e.g., \cite{sun2017remote,tsai2020unifying,ornee2019sampling}) and age of information. 
%In \cite{sun2017remote}, the authors design an optimal sampling policy of Wiener process to minimize the long-term average MMSE. The study in \cite{tsai2020unifying} derives joint sensor and controller waiting policies in Wiener process and shows that in certain scenarios, the optimal joint sampling policy can outperform sensor-only or controller-only schemes e.g., \cite{sun2017remote}. The paper in \cite{ornee2019sampling} studies the OU process which is a limiting case of Wiener process in \cite{sun2017remote}. 



==> sections/useless.tex <==
%\subsection{Proof of Lemma \ref{bellman-optimal}}\label{bellman-optimalapp}
%Our MDP problem has a continuous state space and action space with unbounded cost. However, we can utilize the technique from discrete cases with unbounded cost, such as \cite{sennott1986new,sennott1989average,ross1996stochastic}. 

%(1) 
%The inequality $J(y) \ge \inf_{z\in [0,s]} \mathbb{E} \left[  C(y,z,Y_{i,1}) + \alpha J(\Delta_2) \right]$ is shown in \cite[proof of Theorem 2.1, pg. 31]{ross1996stochastic}. We know show the inverse which is a slight change of \cite[proof of Theorem 2.1, pg. 31]{ross1996stochastic}.

%Since $[0,s]$ is compact, for all $\epsilon>0$, there exists $z_0\in [0,s]$ such that 
%\begin{equation}
%\mathbb{E} \left[  C(y,z_0,Y_{i,1}) + \alpha J(\Delta_2)  \right] \le \inf_{z\in [0,s]} \mathbb{E} \left[  C(y,z,Y_{i,1}) + \alpha J(\Delta_2) \right]+\alpha\epsilon.
%\end{equation}
%Let the policy $f$ chooses $z_0$ at stage $1$, and as it enters a state $\Delta_2$ at stage $2$, it follows a policy such that $J_f(\Delta_2)\le J(\Delta_2)+\epsilon$.
%Hence, 
%\begin{align}
%J_f(y) = & \mathbb{E} \left[  C(y,z_0,Y_{i,1}) + \alpha J_f(\Delta_2)  \right]  \\
%\le &  \mathbb{E} \left[  C(y,z_0,Y_{i,1}) + \alpha J_f(\Delta_2)  \right]  +\alpha\epsilon \\
%\le &  \inf_{z\in [0,s]} \mathbb{E} \left[  C(y,z,Y_{i,1}) + \alpha J(\Delta_2) \right]+ 2\alpha\epsilon.
%\end{align}
%Since $J(y)\le J_f(y)$, let $\epsilon \rightarrow 0$, we get 
%\begin{equation}
%J(y) \le \inf_{z\in [0,s]} \mathbb{E} \left[  C(y,z,Y_{i,1}) + \alpha J(\Delta_2) \right].
%\end{equation}

%Similar technique is also used in 

%(2) is shown directly from \eqref{discount}.

%(3) is a slight change of \cite[proof of Proposition 3]{sennott1986new}.
%For a stationary and deterministic policy $f$, we define an operater $T_f$ on a function $u$ such that 
%\begin{equation}
%(T_f u)(y) =  \mathbb{E} \left[  C(y,f(y),Y_{i,1}) +\alpha u(\Delta_2) \right].
%\end{equation}
%It is clear that: 

%(i), For all functions u,v, $u\le v$ implies $T_f\le T_f v$. 

%(ii) $T_f J_f = J_f$, where $J_f$ is the value function under $f$. This comes directly from Lemma \ref{bellman-optimal} (2).

%(iii) $T_f^n 0 \rightarrow J_f$ as $n\rightarrow \infty$. To see (iii), note that $T_f^n 0(y)$ is equal to $n$-state expected $\alpha$-discounted return under $f$, and this converges to $J_f(y)$ by Lemma \ref{lemma-finite} (1).

%(iv) $T_f^n (-\lambda) \rightarrow J_f$ as $n\rightarrow \infty$, where $-\lambda$ is the lower bound of value functions and is defined in Lemma \ref{lemma-finite}. To see (iv), note that $T_f^n (-\lambda)(y)$ is equal to $n$-state expected $\alpha$-discounted return under $f$ minus $\alpha^n \lambda$, and $\alpha^n \lambda\rightarrow 0$ as $n\rightarrow 0$.

%Suppose the stationary and deterministic policy $f$ satisfies \eqref{bellman}. By (i), (ii) and Lemma \ref{bellman-optimal} (2), $T_f (-\lambda) \le T_f(J) = J\le J_f$. Hence, $T^n_f (-\lambda)\le J$. However, by (iv), $T_f^n (-\lambda) \rightarrow J_f \ge J$. Therefore, $J_f = J$, and $f$ is optimal. 


%===============remote estimation one dimension===================

In this subsection, we assume that the samples $O_t$ is an Ornstein-Uhlenbeck (OU) process and the destination is an estimator.
%The technical setting is the same with Section \ref{system-a} except that 
The key difference from previous works e.g., \cite{tsai2020unifying,sun2017remote,ornee2019sampling,klugel2019aoi} is that the estimator not only receives the accurate samples $O_{S_{i,j}}$ at time $S_{i,j}$ but also has an instant noisy observation of the process $O_t$, called $B_t$. %For example, the estimator can estimate the signals from a local sensor through remote cloud and direct observing. %The error-free channel is modeled as a FCFS queue with i.i.d. service times. 
%We also suppose that there is an acknowledgement that is sent back to the sampler with an i.i.d. random delay whenever a sample is delivered. 
%The forward and backward channels have the same setting described in Section \ref{system-a}.
The model for the estimation problem is provided in Fig. \ref{model} as well. Due to the benefit of $B_t$, the optimal estimation error in our study can be reduced.


%The System starts to operate at time $t=0$. We use $S_i$ to denote the generation time of the $i$-th sample, while $D_i$ denote  its delivery time to the estimator. Moreover, we use $Y_i$ to denote the service time of the $i$-th sample, where we have $0<\mathbb{E}[Y]<\infty$ and $D_i=S_i+Y_i$. Let $U(t)=\max{S_i:D_i\leq t}$ be the
%sampling time of the latest received sample at time $t$. The age of information, or simply age, at time $t$ is defined as 
%\begin{equation}
%\Delta(t)=t-U(t).
%\end{equation}
%Since we have $D_{i}\leq D_{i+1}$, $\Delta(t)$ can be expressed as
%\begin{equation}
%\Delta(t)=t-S_i, \text{if}~t\in[D_i,D_{i+1}), i=0,1,2,\ldots
%\end{equation}

The considered OU process  is defined as the solution to the following stochastic differential equation % (SDE)
\begin{equation}
dO_t=-\theta O_t dt+\sigma d W_t,
\end{equation}
where $\theta>0$ is a parameter, and $W_t$ is the Wiener process and we have $\mathbb{E}[W_tW_s]=\min \{s,t \}$ for all $0\leq t,s\leq\infty$. %Note that when $\theta=0$, then $O_t$ is equivalent to a Wiener process. 

The observation process $B_t$ is modeled as 
\begin{equation}
B_t=hO_t+V_t,
\end{equation}
where $h$ is some constant and $V_t$ is a zero mean white noise process such that for all $0\leq t,s\leq\infty$, we have  
\begin{equation}
\mathbb{E}[V_tV_s]= \left\{
 \begin{array}{lll} 
 r & t=s; \\ 0 & t\ne s. 
 \end{array} \right.
\end{equation}
We suppose that $W_t$ and $V_t$ are uncorrelated such that we have $\mathbb{E}[W_tV_s]=0$ for all $0\leq t,s\leq\infty$.

In this work, we use the Kalman filter \cite{ poor2013introduction} as the estimator. At time $t$, the Kalman filter utilizes both the exact sample and noisy observation $B_t$ and provides the minimum mean squared error (MMSE) estimation $\hat{O}_t$. 
%Due to the benefit of $B_t$, the MMSE in our study is reduced compared with \cite{ornee2019sampling}.
Let $n_t\triangleq\mathbb{E}[(O_t-\hat{O}_t)^2]$ as the MMSE of Kalman filter at time $t$. 
%The objective is to seek the optimal sampler that minimizes the long term average MSE. 
% subject to an average sampling-rate constraint, which can be cast as the following problem:
%\begin{align}
%\text{mse}_\text{opt}=&\inf_{\pi\in\Pi}\limsup_{T\to\infty}\frac{1}{T}\mathbb{E}\left[\int_{0}^T P_t dt\right]\label{opt_eq5} \\&
%\text{s.t.} \liminf_{n\to \infty}\frac{1}{n}\mathbb{E}\left[\sum_{i=1}^n (S_{i+1}-S_i)\right]\geq\frac{1}{f_\text{max}},\label{opt_eq6}
%\end{align}
%\begin{align}
%\text{mse}_\text{opt}=&\inf_{\pi\in\Pi}\limsup_{T\to\infty}\frac{1}{T}\mathbb{E}\left[\int_{0}^T P_t dt\right]\label{opt_eq5}
%\end{align}
%where $\text{mse}_\text{opt}$ is the optimum value of \eqref{opt_eq5}, $f_\text{max}$ is the maximum allowed sampling rate, and $\Pi$  represents the set of all causal sampling policies (some condition might be needed here such as regenerative condition, etc.). Note that the objective function in \eqref{opt_eq5} can be rewritten as (due to the regenerative property and renewal theory):
%\begin{equation}
%\limsup_{T\to\infty}\frac{1}{T}\mathbb{E}\left[\int_{0}^T P_t dt\right]=\limsup_{n\to\infty}\frac{\mathbb{E}\left[
%\sum_{i=0}^n\int_{D_i}^{D_{i+1}} P_t dt\right]}{\mathbb{E}[D_n]}.
%\end{equation}
The estimation process works as follows: Once a sample is delivered to the Kalman filter at time $D_{i,M_i}$, the Kalman filter re-initiate itself with the initial condition $n_t=0$ when $t=S_{i,M_i}$ and starts a new estimation session. Then, during the time period $ [D_{i,M_i},D_{i+1,M_{i+1}})$, the Kalman filter uses the observations $B_t$ for $t\ge S_{i,M_i}$ over time to estimate the process $O_t$.

According to \cite{ poor2013introduction}, $n_t$ for $t
\in[D_{i,M_i},D_{i+1,M_{i+1}})$ satisfies the following Riccati differential equation:
\begin{align}
\frac{dn_t}{dt}=-2\theta n_t+\sigma^2-\frac{h^2}{r}n_t^2.\label{rec_eqn}
\end{align}
%Using \eqref{rec_eqn} and the initial condition $P_t=0$, we can derive 
%We derive the closed-form solution for Equation \eqref{rec_eqn} and show that $P_t$ is a non-decreasing function of the age process $\Delta(t)$. 
For simplicity, we denote $\bar{n}$ and $l$ as 
\begin{align}
\bar{n} & =\frac{-\theta r+\sqrt{(\theta r)^2+\sigma^2 rh^2}}{h^2},\\
l & = \frac{h^2}{2\sqrt{(\theta r)^2+\sigma^2 r h^2}}. \label{remote_9}
\end{align} Then, we have
%\section{Main Results}
%We derive $P_t$ in the next lemma.
\begin{proposition}\label{lim1}
For $t\in[D_{i, M_i},D_{i+1,M_{i+1}})$ and $ i=0,1,2,\ldots$, the MMSE $n_t$ is given by
\begin{align}
n_t=\bar{n}-\frac{1}{l+\left(\frac{1}{\bar{n}}-l\right)e^{2\sqrt{\theta^2+\frac{\sigma^2 h^2}{r}}\Delta_t}}, \label{Lem1eq}
\end{align}
where $\Delta_t=t-S_{i,M_i}$. Moreover, $n_t$ is a bounded and increasing function of the age $\Delta_t$.
\end{proposition}
\begin{proof}
We provide the proof sketch here. 
\ifreport
See Appendix \ref{Appendix_A} for details. 
\else
\fi
%Let us define $\bar{P}$ as the steady state solution of \eqref{rec_eqn}, i.e., it is the solution of the following equation:
%\begin{align}
%0=-2\theta P_t+Q-\frac{H^2}{R}P_t^2.\label{rec_eqn_st}
%\end{align}
%Since our model is observable and controllable, we have $\bar{P}>0$. Hence, $\bar{P}$ is given by
%Without loss of generality, we take the positive solution to \eqref{rec_eqn_st}, 
Define $\mu_t = n_t - \bar{n}$, then $\mu_t$ satisfies 
\begin{align}
\frac{d\mu_t}{dt}=-(2\theta +2\frac{h^2}{r}\bar{n}) \mu_t-\frac{h^2}{r}\mu_t^2.\label{rec_eqn3}
\end{align}
The differential Equation \eqref{rec_eqn3} is a Bernoulli equation and the closed-from solution to \eqref{Lem1eq} can be derived accordingly. 
Note that $1/\bar{n}-l>0$, thus, $n_t$ is a non-decreasing function of the age $\Delta_t$.
\end{proof}
%As a result of Lemma \ref{lim1}, we can use \cite{sun2017update} directly to solve our sampling Problem. 
Therefore, given the extra knowledge of $B_t$ over time, the MMSE is still the closed-form function of the age.
As a result of Proposition \ref{lim1}, when the sampling times $S_{i,j}$ are independent of $O_t$, the MMSE $n_t$ is still a function of age $\Delta_t$. When $S_{i,j}$ are related with causal information of $O_t$, then $n_t$ is not necessary a function of $\Delta_t$.

%Next, we validate Theorem \ref{lim1} by considering 
In the special case, when the side observation has zero knowledge of process $O_t$, i.e., $h=0$ for $t\ge 0$, then the estimator $\hat{O_t}$ is equal to that in \cite{ornee2019sampling}.
Therefore, Proposition \ref{lim1} reduces to \cite[Lemma 4]{ornee2019sampling}:  

%\begin{lemma}\label{Lim2}
the MMSE $n_t$ for $t\in[D_{i,M_i}, D_{i+1,M_{i+1}})$ and $i=0,1,2 ,\ldots$ is given by
\begin{align}
n_t=\frac{\sigma^2}{2\theta}\left(1-e^{-2\theta\Delta_t}\right).\label{Lim2_eq}
\end{align}
Moreover, $n_t$ for $h=0$ is a bounded and increasing function of age $\Delta_t$.
%(b) When $H=0$ and $\theta=0$, the MMSE $P_t$ for $t\in[D_{i,M_i}, D_{i+1,M_{i+1}})$ and $i=0,1,2 ,\ldots$ is given by $P_t=\sigma^2 \Delta_t$.
%\end{lemma}
%Note that Lemma \ref{Lim2} agrees with \cite[Lemma 4]{ornee2019sampling}. When $H=0$, the estimator $\hat{O_t}$ is equal to that in \cite{ornee2019sampling} %for $\theta>0$ and \cite{sun2017remote} for $\theta=0$. 
%Thus, when $H=0$, the problem reduces to the remote estimation problems with signal independence case in \cite{ornee2019sampling}.










